The MAGICAL Benchmark for Robust Imitation

Imitation Learning (IL) algorithms are typically evaluated in the same environment that was used to create demonstrations. This rewards precise reproduction of demonstrations in one particular environment, but provides little information about how robustly an algorithm can generalise the demonstrator's intent to substantially different deployment settings. This paper presents the MAGICAL benchmark suite, which permits systematic evaluation of generalisation by quantifying robustness to different kinds of distribution shift that an IL algorithm is likely to encounter in practice. Using the MAGICAL suite, we confirm that existing IL algorithms overfit significantly to the context in which demonstrations are provided. We also show that standard methods for reducing overfitting are effective at creating narrow perceptual invariances, but are not sufficient to enable transfer to contexts that require substantially different behaviour, which suggests that new approaches will be needed in order to robustly generalise demonstrator intent. Code and data for the MAGICAL suite is available at https://github.com/qxcv/magical/.

==> sections/app-extra.tex <==

\section{Definitions / types (AC, discussion on 2020-04-07)}
The benchmark suite will provide a set of 
\begin{itemize}
    \item Training datasets $D_i$ for $i = 1,\ldots, 5$.  An element $s \in D_i$ is called a \emph{training scenario}.
    \item Testing datasets $T_{i,j}$ for $i=1,\ldots 5$ and $j = 1, \ldots N_i$.  An element $s \in T_{i,j}$ is called a \emph{test scenario}.
\end{itemize}

For example, a training or testing scenario $s$ could be an episode of a reinforcement learning task, like ``put the red blocks at the top of the screen.''

We view a learning algorithm $L$ as any program which can read a dataset $D_i$ and return an agent (or classifier) $A_i = L(D_i)$.  We view an agent $A$ as a program that can interacts with a training or test scenario $s$ to receive a score, denoted by 
\[score(A,s),\]

which is always normalized to range from 0 to 1 as A varies.

The \emph{overall performance} of a learning algorithm $L$ on the benchmark suite $(D_\bullet, T_\bullet)$ is defined as the vector

\[
OP := average_{i,j,s \in T_{i,j}} score(L(D_i),s)
\]

The \emph{compositve performance} of $L$ is just vector of entries in the average computer above as $i$ and $j$ vary, i.e. [...]

\subsection{Sam's notes from last time}

\textbf{Sam:} things to do for next week:
%
\begin{itemize}
    \item An abstract (just compress the framing section below).

    \item ``Type signature'' of the benchmark suite.
    %
    What does a task consist of?
    %
    A configuration?
    %
    etc.

    \item Abstract description of each source of auxiliary data (algorithms don't have to be nailed down).
    %
    A useful way of expressing this would be to say precisely which elements of the benchmark they get access to at training time, and which elements of the benchmark they get access to at testing time.
    %
    Can then explain how those different elements are likely to be useful.

    \item Experiment setup.
    %
    What algorithms am I evaluating?
    %
    What data and training resources do they have acccess to?
    %
    etc.
\end{itemize}
%
Things that I don't need to have done: intro/conclusion, related work, actual experiment results, precise definitions of baseline algorithms, most figures.

\section{Full list of algorithmic techniques to try}

\subsection{Manually-specified invariances (e.g. task-specific inductive biases)}

\begin{itemize}
    \item \textbf{Image augmentations:} small rotations; small translations; small changes in intensity, hue, etc.; Gaussian noise; salt-and-pepper noise; randomly masking out sections of the image.
    %
    These apply to both BC (policy only) and GAIL (policy and discriminator).
    %
    See e.g. task-relevant IL paper for some other ideas (and evidence of the importance of augmentations in GAIL!)~\cite{zolna2019task}.
    
    \item \textbf{Relational bias:} use MHDPA-based architecture from relational RL paper~\cite{zambaldi2018relational}.
    %
    In theory this should be useful for cluster-colour/cluster-type/match-regions tasks, which all require some form of relational reasoning between visual elements in the scene.
    
    \item \textbf{Translational invariance or non-invariance:} can increase translational invariance with, e.g., max or average pooling at flattening layer of the convnet.
    %
    Can also go the other way and add CoordConv to ensure that layers are \textit{not} translationally invariant.
    
    \item \textbf{Hand-segmentation of features:} In principle, I could split the input images out into separate planes for each object attribute (object presence, object colour, object shape, robot location, robot orientation, gripper position, etc. etc.) and pass them straight into the network.
    %
    This would probably make it easier to learn the required invariances, and might also provide a useful baseline.
\end{itemize}

\subsection{Using $k$ demonstrations for one task (large demonstration set)}

\begin{itemize}
    \item \textbf{The obvious thing:} \ldots{}is to throw all of the demonstrations in to whatever algorithm you're using.
    %
    In the analysis, we should still experiment with constraining the number of demonstrations.

    \item \textbf{Option-learning:} with more data, it should be possible to learn low-level options to constrain RL or make it faster.
    %
    This is described in the next section.
    
    \item \textbf{Domain adaptation tricks and IRM/ICP:} Having multiple demonstrations for the same task is useful because the variation between demonstrations can indicate what features are important to task completion and what features are not important.
    %
    As such, when doing GAIL or IRL, we might expect the learnt reward function to behave similarly across each demonstration.
    %
    We could enforce this property by adding a domain adaptation loss to make the marginal distribution of internal activation in the reward network independent of the demo trajectory being processed~\cite{ganin2014unsupervised}.
    %
    We could also use IRM to throw out abstract features that are more useful for classifying some trajectories than others~\cite{arjovsky2019invariant}.
    %
    IRM would arguably be preferable to domain adaptation because it allows the activation distribution to differ between trajectories, so long as the individual features at the last layer of the network are about equally informative for predicting actions in each trajectory.
\end{itemize}

\subsection{Using $k \not\gg 1$ demonstrations for $n$ tasks (multi-task data)}

\begin{itemize}
    \item \textbf{Multi-task learning:} learn multi-headed networks with a common body and task-specific heads.
    %
    Simultaneously train the network and all of its heads on all tasks; this technique applies to both BC (policy only) and GAIL (both policy and discriminator).
    %
    Ideally this should give the network good representations of visual elements that it may not have access to in some tasks.
    %
    For example, if a blue block is present in the ``match regions'' task but not the ``move to corner'' task, then the algorithm should still be able to learn a representation of blue blocks for the ``move to corner'' policy.

    \item \textbf{Option-learning:} Throw all of the available data into an algorithm for learning alternative action space representations or short-horizon plan representations, such as ``look-then-listen''~\cite{gaddy2019pre} or LLPfP~\cite{lynch2019learning}.
    %
    Ideally, these representations should capture primitives like ``grasp the block of shape $x$ and colour $y$'', or ``push the block in direction $z$ without letting go''.
    %
    Because the representations are trained on multi-task data, they should work with a reasonable variety of data.
    %
    Using the resulting representation as a high-level action space for an IL algorithm should therefore make it easier to generalise, since only the high-level policy will encounter any sort of domain gap.
\end{itemize}

\subsection{Using test variants without associated demonstrations (test-time adaptation)}

\begin{itemize}
    \item \textbf{Co-train policy in GAIL:} do RL in the test environment using the discriminator learnt in the training environment, while simultaneously updating the discriminator using data from the training environment.
    %
    This should be effective at transferring invariances from the discriminator to the policy, assuming the discriminator already has the right invariances.
    %
    It would also be possible to freeze the discriminator and then transfer to the test environment, but I don't expect that to work as well.

    \item \textbf{Ensure the GAIL classifier is still discriminative on the test task:} intuitively, we might expect a learnt reward function/discriminator to be roughly equally discriminative between training and testing tasks.
    %
    At the very least, this should be true in the sense that it is possible for policies to achieve a similar range of returns between the two environments.
    %
    We could enforce this by doing GAIL co-training, then adding a loss term like the following to the discriminator:
    %
    \[
        \expect_{\substack{\tau \sim \pi_{\text{n}} \text{ on } \mathcal T_1 \\ \tau' \sim \pi_{\text{n}} \text{ on } \mathcal T_2}}[(\log D_\theta(\tau) - \log D_\theta(\tau'))^2]~,
    \]
    %
    where $\pi_n$ is the novice policy being optimised by GAIL, $\mathcal T_1$ is the first task (with a labelled demonstration), and $\mathcal T_2$ is the second task (without a labelled demonstration).
    %
    This loss could be extended by defining a family of based on the novice policy and ensuring that they all attain similar return; for instance, making sure the return profiles are similar when noise is added to the policy in the train task and in the test task.
    %
    There are probably better/more principled ways of formalising this basic intuition, however.
    
    % \item \textbf{Assume that the demonstrator is well-adapted to the test environment:} \textbf{TODO}

    \item \textbf{Learn options:} use DIAYN or similar to learn low-level options from rollouts in all environments, including the test environment.
    %
    Use the resulting options to learn a high-level policy, or to accelerate exploration (e.g. by randomly excuting options to generate experience for Q-learning).
    
    % \item \textbf{Learn a CycleGAN:} 
\end{itemize}

















%%%%%% SEMI-IMPORTANT INFO THAT I KEPT FROM STYLE FILE %%%%%%

% Papers to be submitted to NeurIPS 2020 must be prepared according to the
% instructions presented here. Papers may only be up to eight pages long,
% including figures. Additional pages \emph{containing only a section on the broader impact, acknowledgments and/or cited references} are allowed. Papers that exceed eight pages of content will not be % reviewed, or in any other way considered for
% presentation at the conference.

% The \verb+natbib+ package will be loaded for you by default.  Citations may be
% author/year or numeric, as long as you maintain internal consistency.  As to the
% format of the references themselves, any style is acceptable as long as it is
% used consistently.
% Of note is the command \verb+\citet+, which produces citations appropriate for
% use in inline text.  For example,

% \begin{figure}
%   \centering
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Sample figure caption.}
% \end{figure}

% Fonts were the main cause of problems in the past years. Your PDF file must only
% contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
% achieve this.

% \section*{Broader Impact}
%
% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.
%
% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

% \begin{ack}
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare 
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.
% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
% \end{ack}

% \section*{References}
%
% References follow the acknowledgments. Use unnumbered first-level heading for
% the references. Any choice of citation style is acceptable as long as you are
% consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
% when listing the references.
% {\bf Note that the Reference section does not count towards the eight pages of content that are allowed.}
% \medskip
% 
% \small

